Deep Perm-Set Net: Learn to predict sets with unknown permutation and cardinality using deep neural networks

Many real-world problems, e.g. object detection, have outputs that are naturally expressed as sets of entities. This creates a challenge for traditional deep neural networks which naturally deal with structured outputs such as vectors, matrices or tensors. We present a novel approach for learning to predict sets with unknown permutation and cardinality using deep neural networks. Specifically, in our formulation we incorporate the permutation as unobservable variable and estimate its distribution during the learning process using alternating optimization. We demonstrate the validity of this new formulation on two relevant vision problems: object detection, for which our formulation outperforms state-of-the-art detectors such as Faster R-CNN and YOLO, and a complex CAPTCHA test, where we observe that, surprisingly, our set based network acquired the ability of mimicking arithmetics without any rules being coded.

==> background.tex <==
\section{Background }
\label{background}

To better explain our approach, we first review some basic background on finite set statistics. 

A random finite set (RFS) $\calY$ is a finite-set valued random variable $\calY=\left\{\by_1,\cdots,\by_m\right\},  m\in\mathbb{N}^*$. The main difference between an RFS and a random vector is that for the former, the number of constituent variables, $m$, is random and the variables themselves are random and unordered. A statistical function describing a finite-set variable $\calY$ is a
combinatorial probability density function $p(\calY)$ which consists of a discrete probability distribution, the so-called cardinality distribution, and a family of joint probability densities on the values of the constituent variables in a set with a fixed cardinality~\cite{mahler2007statistical,vo2017model}, \ie
\begin{equation}
p(\calY) = p(m)U^m p_m(\{\by_{1},\by_{2},\cdots,\by_{m}\})
\label{eq:setprob}
\end{equation} 

 where $p(m)$ is the cardinality distribution of the set $\calY$ and  $p_m(\{\by_{1},\by_{2},\cdots,\by_{m}\})$ is a symmetric joint probability density distribution of the set given known cardinality $m$. $U$ is the unit of hyper-volume in the feature space, which
cancels out the unit of the probability density
$p_m(\cdot)$ making it unit-less, and thereby avoids the unit
mismatch across the different dimensions (cardinalities). 

Finite Set Statistics
provides powerful and practical mathematical tools for dealing with random finite sets, based on the notion
of integration and density that is consistent with the point process theory~\cite{mahler2007statistical}. For example, similar to the definition of a probability density function (PDF) for a random variable, the PDF of an RFS must sum to unity over all possible cardinality values and all possible element values as well as their permutations. This type of statistics, which is derived from the point process stochastic process, defines basic
mathematical operations on finite sets such as functions, derivatives and integrations as well as other statistical
tools such as probability density function of a random finite set and its statistical moments~\cite{mahler2007statistical,vo2017model}.   For
further detail on point processes, we refer the reader to
textbooks such as~\cite{chiu2013stochastic,daley2007introduction,moller2003statistical}.


Conventional machine learning approaches, including the existing deep  networks, have been proposed to learn the optimal parameters $\bw^*$ of the distribution $p(Y|\bx,\bw^*)$ which maps a structured input $\bx$, \eg a tensor, to a structured \emph{output vector} $Y$.
%   
In this paper, we instead propose an approach that can learn the parameters $\bw^*$ for a set distribution that allows one to output an arbitrary \emph{set} $\calY$, \ie  $p(\calY|\bx,\bw^*)$. 
